Dictionary-based Monitoring of Premature Ventricular Contractions: An Ultra-Low-Cost Point-of-Care Service

While cardiovascular diseases (CVDs) are prevalent across economic strata, the economically disadvantaged population is disproportionately affected due to the high cost of traditional CVD management. Accordingly, developing an ultra-low-cost alternative, affordable even to groups at the bottom of the economic pyramid, has emerged as a societal imperative. Against this backdrop, we propose an inexpensive yet accurate home-based electrocardiogram(ECG) monitoring service. Specifically, we seek to provide point-of-care monitoring of premature ventricular contractions (PVCs), high frequency of which could indicate the onset of potentially fatal arrhythmia. Note that a traditional telecardiology system acquires the ECG, transmits it to a professional diagnostic centre without processing, and nearly achieves the diagnostic accuracy of a bedside setup, albeit at high bandwidth cost. In this context, we aim at reducing cost without significantly sacrificing reliability. To this end, we develop a dictionary-based algorithm that detects with high sensitivity the anomalous beats only which are then transmitted. We further compress those transmitted beats using class-specific dictionaries subject to suitable reconstruction/diagnostic fidelity. Such a scheme would not only reduce the overall bandwidth requirement, but also localising anomalous beats, thereby reducing physicians' burden. Finally, using Monte Carlo cross validation on MIT/BIH arrhythmia database, we evaluate the performance of the proposed system. In particular, with a sensitivity target of at most one undetected PVC in one hundred beats, and a percentage root mean squared difference less than 9% (a clinically acceptable level of fidelity), we achieved about 99.15% reduction in bandwidth cost, equivalent to 118-fold savings over traditional telecardiology.

==> AIM_ref <==
% This file was created with JabRef 2.10.
% Encoding: Cp1252

@Article{rubinstein,
  title={Efficient implementation of the K-SVD algorithm using batch orthogonal matching pursuit},
  author={Rubinstein, Ron and Zibulevsky, Michael and Elad, Michael},
  journal={CS Technion},
  volume={40},
  number={8},
  pages={1--15},
  year={2008}
}


@Article{adamo,
  Title                    = {ECG compression retaining the best natural basis k-coefficients via sparse decomposition},
  Author                   = {Adamo, Alessandro and Grossi, Giuliano and Lanzarotti, Raffaella and Lin, Jianyi},
  Journal                  = {Biomedical Signal Processing and Control},
  Year                     = {2015},
  Pages                    = {11--17},
  Volume                   = {15},

  Publisher                = {Elsevier}
}

@Article{ksvd,
  Title                    = {K-SVD: An Algorithm for Designing Overcomplete Dictionaries for Sparse Representation},
  Author                   = {Aharon, Michal and Elad, Michael and Bruckstein, Alfred},
  Journal                  = {IEEE Transactions on signal processing},
  Year                     = {2006},
  Number                   = {11},
  Pages                    = {4311--4322},
  Volume                   = {54},

  Publisher                = {IEEE}
}

@InCollection{amatriain,
  Title                    = {Data mining methods for recommender systems},
  Author                   = {Amatriain, Xavier and Jaimes, Alejandro and Oliver, Nuria and Pujol, Josep M},
  Booktitle                = {Recommender Systems Handbook},
  Publisher                = {Springer},
  Year                     = {2011},
  Pages                    = {39--71}
}

@Article{MCCV,
  Title                    = {A survey of cross-validation procedures for model selection},
  Author                   = {Arlot, Sylvain and Celisse, Alain and others},
  Journal                  = {Statistics surveys},
  Year                     = {2010},
  Pages                    = {40--79},
  Volume                   = {4},

  Publisher                = {The author, under a Creative Commons Attribution License}
}

@Article{baman,
  Title                    = {Relationship between burden of premature ventricular complexes and left ventricular function},
  Author                   = {Baman, Timir S and Lange, Dave C and Ilg, Karl J and Gupta, Sanjaya K and Liu, Tzu-Yu and Alguire, Craig and Armstrong, William and Good, Eric and Chugh, Aman and Jongnarangsin, Krit and others},
  Journal                  = {Heart Rhythm},
  Year                     = {2010},
  Number                   = {7},
  Pages                    = {865--869},
  Volume                   = {7},

  Publisher                = {Elsevier}
}

@InProceedings{bortolan,
  Title                    = {Comparison of four methods for premature ventricular contraction and normal beat clustering},
  Author                   = {Bortolan, G and Jekova, I and Christov, I},
  Booktitle                = {Computers in Cardiology, 2005},
  Year                     = {2005},
  Organization             = {IEEE},
  Pages                    = {921--924}
}

@Article{cha,
  Title                    = {Premature Ventricular Contraction-Induced Cardiomyopathy A Treatable Condition},
  Author                   = {Cha, Yong-Mei and Lee, Glenn K and Klarich, Kyle W and Grogan, Martha},
  Journal                  = {Circulation: Arrhythmia and Electrophysiology},
  Year                     = {2012},
  Number                   = {1},
  Pages                    = {229--236},
  Volume                   = {5},

  Publisher                = {Am Heart Assoc}
}

@InProceedings{HC14,
  Title                    = {Reliable low-cost telecardiology: High-sensitivity detection of ventricular beats using dictionaries},
  Author                   = {Chandra, Bollepalli S and Sastry, Challa S and Jana, Soumya},
  Booktitle                = {e-Health Networking, Applications and Services (Healthcom), 2014 IEEE 16th International Conference on},
  Year                     = {2014},
  Organization             = {IEEE},
  Pages                    = {305--310}
}

@Article{chazal,
  Title                    = {A patient-adapting heartbeat classifier using ECG morphology and heartbeat interval features},
  Author                   = {de Chazal, Philip and Reilly, Richard B},
  Journal                  = {IEEE Transactions on Biomedical Engineering},
  Year                     = {2006},
  Number                   = {12},
  Pages                    = {2535--2543},
  Volume                   = {53},

  Publisher                = {IEEE}
}

@Article{aami,
  Title                    = {Testing and reporting performance results of cardiac rhythm and ST segment measurement algorithms},
  Author                   = {EC57, ANSI-AAMI},
  Journal                  = {Association for the Advancement of Medical Instrumentation, Arlington, VA},
  Year                     = {1998}
}

@Book{elad,
  Title                    = {Sparse and Redundant Representations: From Theory to Applications in Signal and Image Processing},
  Author                   = {Elad, Michael},
  Publisher                = {Springer Publishing Company, Incorporated},
  Year                     = {2010},
  Edition                  = {1st},

  ISBN                     = {144197010X, 9781441970107}
}

@Article{fira1,
  Title                    = {An ECG signals compression method and its validation using NNs},
  Author                   = {Fira, Catalina Monica and Goras, Liviu},
  Journal                  = {IEEE Transactions on Biomedical Engineering},
  Year                     = {2008},
  Number                   = {4},
  Pages                    = {1319--1326},
  Volume                   = {55},

  Publisher                = {IEEE}
}

@Book{gertsch,
  Title                    = {The ECG: a two-step approach to diagnosis},
  Author                   = {Gertsch, Marc},
  Publisher                = {Springer Science \& Business Media},
  Year                     = {2003}
}

@Article{physionet,
  Title                    = {Physiobank, physiotoolkit, and physionet components of a new research resource for complex physiologic signals},
  Author                   = {Goldberger, Ary L and Amaral, Luis AN and Glass, Leon and Hausdorff, Jeffrey M and Ivanov, Plamen Ch and Mark, Roger G and Mietus, Joseph E and Moody, George B and Peng, Chung-Kang and Stanley, H Eugene},
  Journal                  = {Circulation},
  Year                     = {2000},
  Number                   = {23},
  Pages                    = {e215--e220},
  Volume                   = {101},

  Publisher                = {Am Heart Assoc}
}

@Article{hinkle,
  Title                    = {The prognostic significance of ventricular premature contractions in healthy people and in people with coronary heart disease.},
  Author                   = {Hinkle, LE and Carver, ST and Argyros, DC},
  Journal                  = {Acta cardiologica},
  Year                     = {1974},
  Pages                    = {5}
}

@Article{palreddy,
  Title                    = {A patient-adaptable ECG beat classifier using a mixture of experts approach},
  Author                   = {Hu, Yu Hen and Palreddy, Surekha and Tompkins, Willis J},
  Journal                  = {IEEE transactions on biomedical engineering},
  Year                     = {1997},
  Number                   = {9},
  Pages                    = {891--900},
  Volume                   = {44},

  Publisher                = {IEEE}
}

@Article{huang,
  Title                    = {WE-CARE: an intelligent mobile telecardiology system to enable mHealth applications},
  Author                   = {Huang, Anpeng and Chen, Chao and Bian, Kaigui and Duan, Xiaohui and Chen, Min and Gao, Hongqiao and Meng, Chao and Zheng, Qian and Zhang, Yingrui and Jiao, Bingli and others},
  Journal                  = {IEEE journal of biomedical and health informatics},
  Year                     = {2014},
  Number                   = {2},
  Pages                    = {693--702},
  Volume                   = {18},

  Publisher                = {IEEE}
}

@InProceedings{ince1,
  Title                    = {Automated patient-specific classification of premature ventricular contractions},
  Author                   = {Ince, Turker and Kiranyaz, Serkan and Gabbouj, Moncef},
  Booktitle                = {2008 30th Annual International Conference of the IEEE Engineering in Medicine and Biology Society},
  Year                     = {2008},
  Organization             = {IEEE},
  Pages                    = {5474--5477}
}

@Article{jana,
  Title                    = {Optimality of KLT for high-rate transform coding of Gaussian vector-scale mixtures: Application to reconstruction, estimation, and classification},
  Author                   = {Jana, Soumya and Moulin, Pierre},
  Journal                  = {IEEE Transactions on Information Theory},
  Year                     = {2006},
  Number                   = {9},
  Pages                    = {4049--4067},
  Volume                   = {52},

  Publisher                = {IEEE}
}

@Article{jaroslawski,
  Title                    = {In eHealth in India today, the nature of work, the challenges and the finances: an interview-based study},
  Author                   = {Jaros{\l}awski, Szymon and Saberwal, Gayatri},
  Journal                  = {BMC medical informatics and decision making},
  Year                     = {2014},
  Number                   = {1},
  Pages                    = {1},
  Volume                   = {14},

  Publisher                = {BioMed Central}
}

@Article{jiang,
  Title                    = {Block-based neural networks for personalized ECG signal classification},
  Author                   = {Jiang, Wei and Kong, Seong G},
  Journal                  = {IEEE Transactions on Neural Networks},
  Year                     = {2007},
  Number                   = {6},
  Pages                    = {1750--1761},
  Volume                   = {18},

  Publisher                = {IEEE}
}

@Article{kiranyaz,
  Title                    = {Real-Time Patient-Specific ECG Classification by 1-D Convolutional Neural Networks},
  Author                   = {Kiranyaz, Serkan and Ince, Turker and Gabbouj, Moncef},
  Journal                  = {IEEE Transactions on Biomedical Engineering},
  Year                     = {2016},
  Number                   = {3},
  Pages                    = {664--675},
  Volume                   = {63},

  Publisher                = {IEEE}
}

@Article{krasteva,
  Title                    = {QRS template matching for recognition of ventricular ectopic beats},
  Author                   = {Krasteva, Vessela and Jekova, Irena},
  Journal                  = {Annals of Biomedical Engineering},
  Year                     = {2007},
  Number                   = {12},
  Pages                    = {2065--2076},
  Volume                   = {35},

  Publisher                = {Springer}
}

@Article{frugal,
  Title                    = {Frugal engineering: An emerging innovation paradigm},
  Author                   = {Kumar, Nirmalya and Puranam, Phanish},
  Journal                  = {Ivey Business Journal},
  Year                     = {2012},
  Number                   = {2},
  Pages                    = {14--16},
  Volume                   = {76}
}

@Article{leehj,
  Title                    = {Ubiquitous healthcare service using Zigbee and mobile phone for elderly patients},
  Author                   = {Lee, Hak Jong and Lee, Sun Hee and Ha, Kyoo-Seob and Jang, Hak Chul and Chung, Woo-Young and Kim, Ju Young and Chang, Yoon-Seok and Yoo, Dong Hyun},
  Journal                  = {International journal of medical informatics},
  Year                     = {2009},
  Number                   = {3},
  Pages                    = {193--198},
  Volume                   = {78},

  Publisher                = {Elsevier}
}

@Book{ICT,
  Title                    = {Quality and Reliability of Telecommunications Infrastructure},
  Author                   = {Lehr, William H},
  Publisher                = {Routledge},
  Year                     = {2013}
}

@Article{Llamedo,
  Title                    = {An automatic patient-adapted ECG heartbeat classifier allowing expert assistance},
  Author                   = {Llamedo, Mariano and Mart{\'\i}nez, Juan Pablo},
  Journal                  = {IEEE Transactions on Biomedical Engineering},
  Year                     = {2012},
  Number                   = {8},
  Pages                    = {2312--2320},
  Volume                   = {59},

  Publisher                = {IEEE}
}

@InProceedings{mairal,
  Title                    = {Online dictionary learning for sparse coding},
  Author                   = {Mairal, Julien and Bach, Francis and Ponce, Jean and Sapiro, Guillermo},
  Booktitle                = {Proceedings of the 26th annual international conference on machine learning},
  Year                     = {2009},
  Organization             = {ACM},
  Pages                    = {689--696}
}

@Article{melgani,
  Title                    = {Classification of electrocardiogram signals with support vector machines and particle swarm optimization},
  Author                   = {Melgani, Farid and Bazi, Yakoub},
  Journal                  = {IEEE Transactions on Information Technology in Biomedicine},
  Year                     = {2008},
  Number                   = {5},
  Pages                    = {667--677},
  Volume                   = {12},

  Publisher                = {IEEE}
}

@Article{mukhopadhyay,
  Title                    = {A lossless ECG data compression technique using ASCII character encoding},
  Author                   = {Mukhopadhyay, Sourav Kumar and Mitra, Sucharita and Mitra, Madhuchhanda},
  Journal                  = {Computers \& Electrical Engineering},
  Year                     = {2011},
  Number                   = {4},
  Pages                    = {486--497},
  Volume                   = {37},

  Publisher                = {Elsevier}
}

@InCollection{NP,
  Title                    = {On the problem of the most efficient tests of statistical hypotheses},
  Author                   = {Neyman, Jerzy and Pearson, Egon S},
  Booktitle                = {Breakthroughs in Statistics},
  Publisher                = {Springer},
  Year                     = {1992},
  Pages                    = {73--108}
}

@Article{ng,
  Title                    = {Treating patients with ventricular ectopic beats},
  Author                   = {Ng, G Andr{\'e}},
  Journal                  = {Heart},
  Year                     = {2006},
  Number                   = {11},
  Pages                    = {1707--1712},
  Volume                   = {92},

  Publisher                = {BMJ Publishing Group Ltd and British Cardiovascular Society}
}

@Article{affordability,
  Title                    = {Practical measurement of affordability: an application to medicines},
  Author                   = {Ni{\"e}ns, LM and Van de Poel, Ellen and Cameron, A and Ewen, M and Laing, R and Brouwer, WBF},
  Journal                  = {Bulletin of the World Health Organization},
  Year                     = {2012},
  Number                   = {3},
  Pages                    = {219--227},
  Volume                   = {90},

  Publisher                = {SciELO Public Health}
}

@Article{niwano,
  Title                    = {Prognostic significance of frequent premature ventricular contractions originating from the ventricular outflow tract in patients with normal left ventricular function},
  Author                   = {Niwano, Shinichi and Wakisaka, Yuko and Niwano, Hiroe and Fukaya, Hidehira and Kurokawa, Sayaka and Kiryu, Michiro and Hatakeyama, Yuko and Izumi, Tohru},
  Journal                  = {Heart},
  Year                     = {2009},
  Number                   = {15},
  Pages                    = {1230--1237},
  Volume                   = {95},

  Publisher                = {BMJ Publishing Group Ltd and British Cardiovascular Society}
}

@Article{page,
  Title                    = {Asymptomatic arrhythmias in patients with symptomatic paroxysmal atrial fibrillation and paroxysmal supraventricular tachycardia.},
  Author                   = {Page, Richard L and Wilkinson, William E and Clair, Walter K and McCarthy, Elisabeth A and Pritchett, EL},
  Journal                  = {Circulation},
  Year                     = {1994},
  Number                   = {1},
  Pages                    = {224--227},
  Volume                   = {89},

  Publisher                = {Am Heart Assoc}
}

@Article{perlmutter,
  Title                    = {Bayes risk weighted vector quantization with posterior estimation for image compression and classification},
  Author                   = {Perlmutter, Keren O and Perlmutter, Sharon M and Gray, Robert M and Olshen, Richard A and Oehler, Karen L},
  Journal                  = {IEEE Transactions on Image Processing},
  Year                     = {1996},
  Number                   = {2},
  Pages                    = {347--360},
  Volume                   = {5},

  Publisher                = {IEEE}
}

@Book{podrid,
  Title                    = {Cardiac arrhythmia: mechanisms, diagnosis, and management},
  Author                   = {Podrid, Philip J and Kowey, Peter R},
  Publisher                = {Lippincott Williams \& Wilkins},
  Year                     = {2001}
}

@Book{BOP,
  Title                    = {The Fortune at the Bottom of the Pyramid},
  Author                   = {Prahalad, Coimbatore Krishna},
  Publisher                = {Pearson Education India},
  Year                     = {2006}
}

@Article{purohit,
  Title                    = {Private initiatives and policy options: recent health system experience in India},
  Author                   = {Purohit, Brijesh C},
  Journal                  = {Health policy and planning},
  Year                     = {2001},
  Number                   = {1},
  Pages                    = {87--97},
  Volume                   = {16},

  Publisher                = {Oxford Univ Press}
}

@Book{sornmo,
  Title                    = {Bioelectrical signal processing in cardiac and neurological applications},
  Author                   = {S{\"o}rnmo, Leif and Laguna, Pablo},
  Publisher                = {Academic Press},
  Year                     = {2005},
  Volume                   = {8}
}

@Article{scheidt,
  Title                    = {Remote electrocardiography: clinical experience with telephone transmission of electrocardiograms},
  Author                   = {Scheidt, Stephen and McGill, Janice and Wilner, Gary and Killip, Thomas},
  Journal                  = {JAMA},
  Year                     = {1974},
  Number                   = {9},
  Pages                    = {1293--1294},
  Volume                   = {230},

  Publisher                = {American Medical Association}
}

@Article{steg,
  Title                    = {ESC Guidelines for the management of acute myocardial infarction in patients presenting with ST-segment elevation},
  Author                   = {Steg, Ph Gabriel and James, Stefan K and Atar, Dan and Badano, Luigi P and Lundqvist, Carina Blomstrom and Borger, Michael A and Di Mario, Carlo and Dickstein, Kenneth and Ducrocq, Gregory and Fernandez-Aviles, Francisco and others},
  Journal                  = {European heart journal},
  Year                     = {2012},
  Pages                    = {ehs215},

  Publisher                = {Eur Soc Cardiology}
}

@Article{tai,
  Title                    = {A 2-D ECG compression method based on wavelet transform and modified SPIHT},
  Author                   = {Tai, Shen-Chuan and Sun, ChiaChun and Yan, Wen-Chien},
  Journal                  = {IEEE Transactions on Biomedical Engineering},
  Year                     = {2005},
  Number                   = {6},
  Pages                    = {999--1008},
  Volume                   = {52},

  Publisher                = {IEEE}
}

@Article{varshney,
  Title                    = {Pervasive healthcare and wireless health monitoring},
  Author                   = {Varshney, Upkar},
  Journal                  = {Mobile Networks and Applications},
  Year                     = {2007},
  Number                   = {2-3},
  Pages                    = {113--127},
  Volume                   = {12},

  Publisher                = {Springer-Verlag New York, Inc.}
}

@Book{vlodaver,
  Title                    = {Coronary Heart Disease: Clinical, Pathological, Imaging, and Molecular Profiles},
  Author                   = {Vlodaver, Zeev and Wilson, Robert F and Garry, Daniel},
  Publisher                = {Springer Science \& Business Media},
  Year                     = {2012}
}

@Article{west,
  Title                    = {How mobile devices are transforming healthcare},
  Author                   = {West, Darrell},
  Journal                  = {Issues in technology innovation},
  Year                     = {2012},
  Number                   = {1},
  Pages                    = {1--11},
  Volume                   = {18}
}

@Article{ye,
  Title                    = {Heartbeat classification using morphological and dynamic features of ECG signals},
  Author                   = {Ye, Can and Kumar, BVK Vijaya and Coimbra, Miguel Tavares},
  Journal                  = {IEEE Transactions on Biomedical Engineering},
  Year                     = {2012},
  Number                   = {10},
  Pages                    = {2930--2941},
  Volume                   = {59},

  Publisher                = {IEEE}
}

@Article{zzhang,
  Title                    = {Heartbeat classification using disease-specific feature selection},
  Author                   = {Zhang, Zhancheng and Dong, Jun and Luo, Xiaoqing and Choi, Kup-Sze and Wu, Xiaojun},
  Journal                  = {Computers in biology and medicine},
  Year                     = {2014},
  Pages                    = {79--89},
  Volume                   = {46},

  Publisher                = {Elsevier}
}

@Article{wdd,
  Title                    = {The weighted diagnostic distortion (WDD) measure for ECG signal compression},
  Author                   = {Zigel, Yaniv and Cohen, Arnon and Katz, Amos},
  Journal                  = {IEEE Transactions on Biomedical Engineering},
  Year                     = {2000},
  Number                   = {11},
  Pages                    = {1422--1430},
  Volume                   = {47},

  Publisher                = {IEEE}
}

@Article{zigel1,
  Title                    = {ECG signal compression using analysis by synthesis coding},
  Author                   = {Zigel, Yaniv and Cohen, Arnon and Katz, Amos},
  Journal                  = {IEEE Transactions on Biomedical Engineering},
  Year                     = {2000},
  Number                   = {10},
  Pages                    = {1308--1316},
  Volume                   = {47},

  Publisher                = {IEEE}
}

@Other{poverty,
  Owner                    = {jagath},
  Timestamp                = {2016.07.17},
  Url                      = {http://data.worldbank.org/indicator/SI.POV.DDAY}
}

@InProceedings{WHO,
  Title                    = {World Health Organization, Fact sheet on CVDs (Fact sheet N${}^{0}$317)},
  Year                     = {2013},
  Month                    = {March},

  Journal                  = {World Health Organization},
  Owner                    = {Kiran},
  Timestamp                = {2014.11.24},
  Url                      = {http://www.who.int/mediacentre/factsheets/fs317/en/}
}



==> Fig_BW.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{BWvsPRD1} \\
\includegraphics[width=0.40\textwidth]{Full_L5} 

%\includegraphics[width=0.45\textwidth]{BandwidthUsageVsR_Se_new} \\
\caption{Three-way tradeoff between bandwidth, sensitivity and $PRD^{ext}$.}
\label{bw}
\end{figure}


==> Fig_Beats.tex <==
\begin{figure}
\centering
\includegraphics[width = 8cm]{Beats3}
\caption{Segmented normal and PVC beat.}
\label{beats}
\end{figure}

==> Fig_CompClass.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{CompClassBlock} \\

%\includegraphics[width=0.45\textwidth]{BandwidthUsageVsR_Se_new} \\
\caption{Simplified compression and classification block.}
\label{CompClass}
\end{figure}


==> Fig_Compression.tex <==
%\begin{figure}[t]
%\centering
%\includegraphics[width=3in]{CompRatioNewEdited}\\
%(a)  \\
%\includegraphics[width=3in]{BandwidthUsageNewEdited}\\
%(b) \\
%\caption{(a) Plot of compression ratio versus $R^2$ score for dictionary sizes 300 and 600; (b) Plot of bandwidth usage versus $R^2$ score.}
%\label{cr}
%\end{figure}

\begin{figure}[]
\centering
\includegraphics[width=3in]{CompRatioComparisionPlot_new}
\caption{Compression ratio versus reconstruction fidelity for Normal and PVC dictionaries.}
\label{cr}
\end{figure}



==> Fig_RecSig.tex <==
%\begin{figure*}[ht]
%\begin{centering}
%\includegraphics[width=5cm]{legend} 
%\begin{tabular}{ccc}
%\includegraphics[width=5.3cm]{RecSig_Rsq91} & \includegraphics[width=5.3cm]{RecSig_Rsq95} & \includegraphics[width=5.3cm]{RecSig_Rsq98}  \\
%\includegraphics[width=5.3cm]{RecErr_Rsq91}  & \includegraphics[width=5.3cm]{RecErr_Rsq95} & \includegraphics[width=5.3cm]{RecErr_Rsq98} \\
%(a) & (b) & (c) \\
%\end{tabular}•
%\caption{Plot of original and recovered signal and their corresponding error for PRD of 9\%, 5\% and 2\% respectively}
%\label{rec}
%\end{centering}
%\end{figure*}

\begin{figure}[ht]
\begin{centering}
\begin{tabular}{c}
\includegraphics[width=8cm]{Org_rec_sig}  \\
(a) \\ 
\includegraphics[width=8cm]{Err_sig}  \\
(b) \\
\end{tabular}
\caption{(a) Plot of original and recovered signals, (b) Corresponding error for PRD of 9\%, 5\% and 2\% respectively}
\label{rec}
\end{centering}
\end{figure}

==> Fig_ppv_se.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{ppv_plot} \\
\caption{ Positve predictive value vs Sensitivity for various PRD values }
\label{ppv_se}
\end{figure}

==> Table_datasets.tex <==
%\begin{table*}[t]
%\renewcommand{\arraystretch}{1.2}
%\centering
%\resizebox{160mm}{!}{
%\begin{tabular}{C{1.5cm}C{10cm}C{1.25cm}C{1.25cm}C{2cm}}
%\hline
%\multicolumn{1}{c}{Label} & \multicolumn{1}{c}{Subject ID in MIT-BIH arrhythmia databased}                                                                                                 & normal beats & PVC beats&Algorithms                                                                                \\ \hline \hline
% \multirow{3}{*}{Set-1}                      & Training: 100, 105, 106, 108, 109, 111, 114, 116, 118, 119, 121, 123 and 124    & 25360 (37\%) & 1281 (18.3\%) & \multirow{2}{*}{Hu} \\ 
%                         & Testing: 200, 201, 202, 203, 205, 207, 208, 209, 210, 213, 124, 215, 219, 221, 223, 228, 230, 231, 233 and 234           &   43130 (63\%) & 5727 (81.7\%) &                                                                                         \\ \hline
% \multirow{3}{*}{Set-2}                          & Training: 101, 106, 108, 109, 112, 114, 115, 116, 118, 119, 122, 124, 201, 203, 205, 207, 208, 209, 215, 220, 223 and 230           &  45843 (50.9\%) & 3788 (54\%) & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Chazal, \\  Llamedo \\ and Zhang\end{tabular}} \\ 
%                         & Testing: 100, 103, 105, 111, 113, 117, 121, 123, 200, 202, 210, 212, 213, 214, 219, 221, 222, 228, 231, 232, 233 and 234           &         44283 (49.1\%) & 3220 (46\%) &                                                                                   \\ \hline
% \multirow{3}{*}{Set-3}                           & Training: 100, 101, 103, 105, 106, 108, 109, 111, 112, 113, 114, 115, 116, 117, 118, 119, 121, 122, 123 and 124                     &   39582 (43.9\%) & 1281 (18.9\%) &    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Jiang, \\ Ince and \\ Kiranyaz\end{tabular}}   \\ 
%                        & Testing: 200, 201, 202, 203, 205, 207, 208, 209, 210, 212, 213, 214, 215, 219, 220, 221, 222, 223, 228, 230, 231, 232, 233 and 234 &       50499 (56.1\%) & 5727 (81.7\%) &                                                                                     \\ \hline
% \multirow{3}{*}{Set-4}                           & Training: 105, 106, 108, 109, 111, 116, 118, 124, 200, 201, 202, 203, 205, 207, 209, 210, 212, 214, 215, 223, 228 and 232           &   45575 50.6\%) & 4008 (57.2\%) &   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}  Proposed\\ algorithm\\ \end{tabular}}  \\ 
%                         & Testing: 100, 101, 103, 112, 113, 114, 115, 117, 119, 121, 122, 123, 208, 213, 219, 220, 221, 222, 230, 231, 233 and 234           &  44506 (49.4\%) & 3000 (42.8\%) &  \\  \hline
%
%Random selection $(^{44}C_{22})$  &  22 out of 44 subjects are randomly chosen to form test set. Experiment is repeated for 100 random selections. &  \multicolumn{2}{C{2.5cm}}{Each test set has 45\%--55\% of total PVC beats} &  Proposed algorithm  \\  \hline
%
%Random selection $(^{44}C_{4})$  &  4 out of 44 subjects are randomly chosen to form test set. Experiment is repeated for 100 random selections. &  \multicolumn{2}{C{2.5cm}}{Each test set has 10\%--20\% of total PVC beats} &  Proposed algorithm  \\ \hline
%
%\end{tabular}}
%
%\caption{Data set partitioning considered in various algorithms}
%\label{data_partition}
%\end{table*}


\begin{table*}[t]
\renewcommand{\arraystretch}{1.2}
\centering
\resizebox{160mm}{!}{
\begin{tabular}{C{1.5cm}C{10cm}C{1.25cm}C{1.25cm}}
\hline
\multicolumn{1}{c}{Set index} & \multicolumn{1}{c}{Subject ID in MIT-BIH arrhythmia databased}                                                                                                 & normal beats & PVC beats                                                                               \\ \hline \hline
 \multirow{3}{*}{Set-1}                      & Training: 100, 105, 106, 108, 109, 111, 114, 116, 118, 119, 121, 123 and 124    & 25360 (37\%) & 1281 (18.3\%)  \\ 
                         & Testing: 200, 201, 202, 203, 205, 207, 208, 209, 210, 213, 124, 215, 219, 221, 223, 228, 230, 231, 233 and 234           &   43130 (63\%) & 5727 (81.7\%)                                                                                        \\ \hline
 \multirow{3}{*}{Set-2}                          & Training: 101, 106, 108, 109, 112, 114, 115, 116, 118, 119, 122, 124, 201, 203, 205, 207, 208, 209, 215, 220, 223 and 230           &  45843 (50.9\%) & 3788 (54\%) \\ 
                         & Testing: 100, 103, 105, 111, 113, 117, 121, 123, 200, 202, 210, 212, 213, 214, 219, 221, 222, 228, 231, 232, 233 and 234           &         44283 (49.1\%) & 3220 (46\%)                                                                                 \\ \hline
 \multirow{3}{*}{Set-3}                           & Training: 100, 101, 103, 105, 106, 108, 109, 111, 112, 113, 114, 115, 116, 117, 118, 119, 121, 122, 123 and 124                     &   39582 (43.9\%) & 1281 (18.9\%)  \\ 
                        & Testing: 200, 201, 202, 203, 205, 207, 208, 209, 210, 212, 213, 214, 215, 219, 220, 221, 222, 223, 228, 230, 231, 232, 233 and 234 &       50499 (56.1\%) & 5727 (81.7\%)                                                                                     \\ \hline
 \multirow{3}{*}{Set-4}                           & Training: 105, 106, 108, 109, 111, 116, 118, 124, 200, 201, 202, 203, 205, 207, 209, 210, 212, 214, 215, 223, 228 and 232           &   45575 50.6\%) & 4008 (57.2\%)  \\ 
                         & Testing: 100, 101, 103, 112, 113, 114, 115, 117, 119, 121, 122, 123, 208, 213, 219, 220, 221, 222, 230, 231, 233 and 234           &  44506 (49.4\%) & 3000 (42.8\%)  \\  \hline

%Random selection $(^{44}C_{22})$  &  22 out of 44 subjects are randomly chosen to form test set. Experiment is repeated for 100 random selections. &  \multicolumn{2}{C{2.5cm}}{Each test set has 45\%--55\% of total PVC beats} &  Proposed algorithm  \\  \hline

%Random selection $(^{44}C_{4})$  &  4 out of 44 subjects are randomly chosen to form test set. Experiment is repeated for 100 random selections. &  \multicolumn{2}{C{2.5cm}}{Each test set has 10\%--20\% of total PVC beats} &  Proposed algorithm  \\ \hline

\end{tabular}}

\caption{Data set partitioning considered in various algorithms}
\label{data_partition}
\end{table*}

==> refer.tex <==
\begin{thebibliography}{100}
\bibliographystyle{elsarticle-num.bst}

\bibitem{WHO}
World health organization, fact sheet on cvds (fact sheet n${}^{0}$317), 2013.

\bibitem{podrid}
P.~J. Podrid, P.~R. Kowey, Cardiac arrhythmia: mechanisms, diagnosis, and
  management, Lippincott Williams \& Wilkins, 2001.

\bibitem{gertsch}
M.~Gertsch, The ECG: a two-step approach to diagnosis, Springer Science \&
  Business Media, 2003.

\bibitem{hinkle}
L.~Hinkle, S.~Carver, D.~Argyros, The prognostic significance of ventricular
  premature contractions in healthy people and in people with coronary heart
  disease., Acta cardiologica (1974) 5.

\bibitem{ng}
G.~A. Ng, Treating patients with ventricular ectopic beats, Heart 92~(11)
  (2006) 1707--1712.

\bibitem{poverty}
\urlprefix\url{http://data.worldbank.org/indicator/SI.POV.DDAY}

\bibitem{west}
D.~West, How mobile devices are transforming healthcare, Issues in technology
  innovation 18~(1) (2012) 1--11.

\bibitem{BOP}
C.~K. Prahalad, The Fortune at the Bottom of the Pyramid, Pearson Education
  India, 2006.

\bibitem{frugal}
N.~Kumar, P.~Puranam, Frugal engineering: An emerging innovation paradigm, Ivey
  Business Journal 76~(2) (2012) 14--16.

\bibitem{palreddy}
Y.~H. Hu, S.~Palreddy, W.~J. Tompkins, A patient-adaptable ecg beat classifier
  using a mixture of experts approach, IEEE transactions on biomedical
  engineering 44~(9) (1997) 891--900.

\bibitem{chazal}
P.~de~Chazal, R.~B. Reilly, A patient-adapting heartbeat classifier using ecg
  morphology and heartbeat interval features, IEEE Transactions on Biomedical
  Engineering 53~(12) (2006) 2535--2543.

\bibitem{Llamedo}
M.~Llamedo, J.~P. Mart{\'\i}nez, An automatic patient-adapted ecg heartbeat
  classifier allowing expert assistance, IEEE Transactions on Biomedical
  Engineering 59~(8) (2012) 2312--2320.

\bibitem{melgani}
F.~Melgani, Y.~Bazi, Classification of electrocardiogram signals with support
  vector machines and particle swarm optimization, IEEE Transactions on
  Information Technology in Biomedicine 12~(5) (2008) 667--677.

\bibitem{jiang}
W.~Jiang, S.~G. Kong, Block-based neural networks for personalized ecg signal
  classification, IEEE Transactions on Neural Networks 18~(6) (2007)
  1750--1761.

\bibitem{ince}
T.~Ince, S.~Kiranyaz, M.~Gabbouj, Automated patient-specific classification of
  premature ventricular contractions, in: 2008 30th Annual International
  Conference of the IEEE Engineering in Medicine and Biology Society, IEEE,
  2008, pp. 5474--5477.

\bibitem{zzhang}
Z.~Zhang, J.~Dong, X.~Luo, K.-S. Choi, X.~Wu, Heartbeat classification using
  disease-specific feature selection, Computers in biology and medicine 46
  (2014) 79--89.

\bibitem{kiranyaz}
S.~Kiranyaz, T.~Ince, M.~Gabbouj, Real-time patient-specific ecg classification
  by 1-d convolutional neural networks, IEEE Transactions on Biomedical
  Engineering 63~(3) (2016) 664--675.

\bibitem{bortolan}
G.~Bortolan, I.~Jekova, I.~Christov, Comparison of four methods for premature
  ventricular contraction and normal beat clustering, in: Computers in
  Cardiology, 2005, IEEE, 2005, pp. 921--924.

\bibitem{tai}
S.-C. Tai, C.~Sun, W.-C. Yan, A 2-d ecg compression method based on wavelet
  transform and modified spiht, IEEE Transactions on Biomedical Engineering
  52~(6) (2005) 999--1008.

\bibitem{zigel1}
Y.~Zigel, A.~Cohen, A.~Katz, Ecg signal compression using analysis by synthesis
  coding, IEEE Transactions on Biomedical Engineering 47~(10) (2000)
  1308--1316.

\bibitem{fira1}
C.~M. Fira, L.~Goras, An ecg signals compression method and its validation
  using nns, IEEE Transactions on Biomedical Engineering 55~(4) (2008)
  1319--1326.

\bibitem{adamo}
A.~Adamo, G.~Grossi, R.~Lanzarotti, J.~Lin, Ecg compression retaining the best
  natural basis k-coefficients via sparse decomposition, Biomedical Signal
  Processing and Control 15 (2015) 11--17.

\bibitem{jana}
S.~Jana, P.~Moulin, Optimality of klt for high-rate transform coding of
  gaussian vector-scale mixtures: Application to reconstruction, estimation,
  and classification, IEEE Transactions on Information Theory 52~(9) (2006)
  4049--4067.

\bibitem{vlodaver}
Z.~Vlodaver, R.~F. Wilson, D.~Garry, Coronary Heart Disease: Clinical,
  Pathological, Imaging, and Molecular Profiles, Springer Science \& Business
  Media, 2012.

\bibitem{cha}
Y.-M. Cha, G.~K. Lee, K.~W. Klarich, M.~Grogan, Premature ventricular
  contraction-induced cardiomyopathy a treatable condition, Circulation:
  Arrhythmia and Electrophysiology 5~(1) (2012) 229--236.

\bibitem{niwano}
S.~Niwano, Y.~Wakisaka, H.~Niwano, H.~Fukaya, S.~Kurokawa, M.~Kiryu,
  Y.~Hatakeyama, T.~Izumi, Prognostic significance of frequent premature
  ventricular contractions originating from the ventricular outflow tract in
  patients with normal left ventricular function, Heart 95~(15) (2009)
  1230--1237.

\bibitem{baman}
T.~S. Baman, D.~C. Lange, K.~J. Ilg, S.~K. Gupta, T.-Y. Liu, C.~Alguire,
  W.~Armstrong, E.~Good, A.~Chugh, K.~Jongnarangsin, et~al., Relationship
  between burden of premature ventricular complexes and left ventricular
  function, Heart Rhythm 7~(7) (2010) 865--869.

\bibitem{scheidt}
S.~Scheidt, J.~McGill, G.~Wilner, T.~Killip, Remote electrocardiography:
  clinical experience with telephone transmission of electrocardiograms, JAMA
  230~(9) (1974) 1293--1294.

\bibitem{varshney}
U.~Varshney, Pervasive healthcare and wireless health monitoring, Mobile
  Networks and Applications 12~(2-3) (2007) 113--127.

\bibitem{huang}
A.~Huang, C.~Chen, K.~Bian, X.~Duan, M.~Chen, H.~Gao, C.~Meng, Q.~Zheng,
  Y.~Zhang, B.~Jiao, et~al., We-care: an intelligent mobile telecardiology
  system to enable mhealth applications, IEEE journal of biomedical and health
  informatics 18~(2) (2014) 693--702.

\bibitem{leehj}
H.~J. Lee, S.~H. Lee, K.-S. Ha, H.~C. Jang, W.-Y. Chung, J.~Y. Kim, Y.-S.
  Chang, D.~H. Yoo, Ubiquitous healthcare service using zigbee and mobile phone
  for elderly patients, International journal of medical informatics 78~(3)
  (2009) 193--198.

\bibitem{Mukhopadhyay}
S.~K. Mukhopadhyay, S.~Mitra, M.~Mitra, A lossless ecg data compression
  technique using ascii character encoding, Computers \& Electrical Engineering
  37~(4) (2011) 486--497.

\bibitem{ICT}
W.~H. Lehr, Quality and Reliability of Telecommunications Infrastructure,
  Routledge, 2013.

\bibitem{steg}
P.~G. Steg, S.~K. James, D.~Atar, L.~P. Badano, C.~B. Lundqvist, M.~A. Borger,
  C.~Di~Mario, K.~Dickstein, G.~Ducrocq, F.~Fernandez-Aviles, et~al., Esc
  guidelines for the management of acute myocardial infarction in patients
  presenting with st-segment elevation, European heart journal (2012) ehs215.

\bibitem{purohit}
B.~C. Purohit, Private initiatives and policy options: recent health system
  experience in india, Health policy and planning 16~(1) (2001) 87--97.

\bibitem{jaroslawski}
S.~Jaros{\l}awski, G.~Saberwal, In ehealth in india today, the nature of work,
  the challenges and the finances: an interview-based study, BMC medical
  informatics and decision making 14~(1) (2014) 1.

\bibitem{physionet}
A.~L. Goldberger, L.~A. Amaral, L.~Glass, J.~M. Hausdorff, P.~C. Ivanov, R.~G.
  Mark, J.~E. Mietus, G.~B. Moody, C.-K. Peng, H.~E. Stanley, Physiobank,
  physiotoolkit, and physionet components of a new research resource for
  complex physiologic signals, Circulation 101~(23) (2000) e215--e220.

\bibitem{affordability}
L.~Ni{\"e}ns, E.~Van~de Poel, A.~Cameron, M.~Ewen, R.~Laing, W.~Brouwer,
  Practical measurement of affordability: an application to medicines, Bulletin
  of the World Health Organization 90~(3) (2012) 219--227.

\bibitem{household}
\urlprefix\url{http://www.nakono.com/tekcarta/databank/households-average-household-size}

\bibitem{NP}
J.~Neyman, E.~S. Pearson, On the problem of the most efficient tests of
  statistical hypotheses, in: Breakthroughs in Statistics, Springer, 1992, pp.
  73--108.

\bibitem{sornmo}
L.~S{\"o}rnmo, P.~Laguna, Bioelectrical signal processing in cardiac and
  neurological applications, Vol.~8, Academic Press, 2005.

\bibitem{wdd}
Y.~Zigel, A.~Cohen, A.~Katz, The weighted diagnostic distortion (wdd) measure
  for ecg signal compression, IEEE Transactions on Biomedical Engineering
  47~(11) (2000) 1422--1430.

\bibitem{elad}
M.~Elad, Sparse and Redundant Representations: From Theory to Applications in
  Signal and Image Processing, 1st Edition, Springer Publishing Company,
  Incorporated, 2010.

\bibitem{rubinstein}
R.~Rubinstein, M.~Zibulevsky, M.~Elad, Efficient implementation of the k-svd
  algorithm using batch orthogonal matching pursuit, CS Technion 40~(8) (2008)
  1--15.

\bibitem{ksvd}
M.~Aharon, M.~Elad, A.~Bruckstein, K-svd: An algorithm for designing
  overcomplete dictionaries for sparse representation, IEEE Transactions on
  signal processing 54~(11) (2006) 4311--4322.

\bibitem{haykin}
S.~Haykin, Communication systems, John Wiley \& Sons, 2008.

\bibitem{ye}
C.~Ye, B.~V. Kumar, M.~T. Coimbra, Heartbeat classification using morphological
  and dynamic features of ecg signals, IEEE Transactions on Biomedical
  Engineering 59~(10) (2012) 2930--2941.

\bibitem{krasteva}
V.~Krasteva, I.~Jekova, Qrs template matching for recognition of ventricular
  ectopic beats, Annals of Biomedical Engineering 35~(12) (2007) 2065--2076.

\bibitem{aami}
A.-A. EC57, Testing and reporting performance results of cardiac rhythm and st
  segment measurement algorithms, Association for the Advancement of Medical
  Instrumentation, Arlington, VA.

\bibitem{HC14}
B.~S. Chandra, C.~S. Sastry, S.~Jana, Reliable low-cost telecardiology:
  High-sensitivity detection of ventricular beats using dictionaries, in:
  e-Health Networking, Applications and Services (Healthcom), 2014 IEEE 16th
  International Conference on, IEEE, 2014, pp. 305--310.

\bibitem{MCCV}
S.~Arlot, A.~Celisse, et~al., A survey of cross-validation procedures for model
  selection, Statistics surveys 4 (2010) 40--79.

\bibitem{page}
R.~L. Page, W.~E. Wilkinson, W.~K. Clair, E.~A. McCarthy, E.~Pritchett,
  Asymptomatic arrhythmias in patients with symptomatic paroxysmal atrial
  fibrillation and paroxysmal supraventricular tachycardia., Circulation 89~(1)
  (1994) 224--227.

\bibitem{mairal}
J.~Mairal, F.~Bach, J.~Ponce, G.~Sapiro, Online dictionary learning for sparse
  coding, in: Proceedings of the 26th annual international conference on
  machine learning, ACM, 2009, pp. 689--696.

\end{thebibliography}


==> referencesNew.tex <==
%\section*{References}

\begin{thebibliography}{100}
\bibliographystyle{harvard}
%\bibliographystyle{IEEEtran}

%\bibitem{gupta} R. Gupta and M. Mitra, ``Wireless electrocardiogram transmission in ISM band: an approach towards telecardiology." {\em Journal of medical systems,} vol. 38, no. 10, pp. 1-14, 2014.

%\bibitem{stats} {\url http://www.un.org/en/globalissues/briefingpapers/food/vitalstats.shtml}

\bibitem{WHO} World Health Organization, Cardiovascular diseases (CVDs), Fact sheet $N^{0}317$, March 2013.

%\bibitem{thygesen} K. Thygesen, J. S. Alpert and H. D. White, ``Universal definition of myocardial infarction," {\em Journal of the American College of Cardiology,} vol. 50, no. 22, pp. 2173--2195, 2007.

%\bibitem{schunkert} H. Schunkert, U. Broeckel,H. W. Hense, U. Keil and G. A. Riegger, ``Left-ventricular dysfunction," {\em The Lancet,} vol. 351, no. 9099, pp. 372, 1998.

\bibitem{podrid} P. J. Podrid and P. R. Kowey (editors), {\em Cardiac arrhythmia: mechanisms, diagnosis, and management,} Lippincott, Williams \& Wilkins, 2001.

\bibitem{gertsch} M. Gertsch, ``Ventricular Premature Beats," {\em The ECG,} pp. 435-444, Springer, Berlin, 2004.

\bibitem{hinkle} L. E. Hinkle, S. T. Carver and D. C. Argyros, ``The prognostic significance of ventricular premature contractions in healthy people and in people with coronary heart disease," {\em Acta cardiologica,} pp. 5, 1974.

\bibitem{cha} Y. M. Cha, G. K. Lee, K. W. Klarich and M. Grogan, ``Premature Ventricular Contraction-Induced Cardiomyopathy A Treatable Condition," {\em Circulation: Arrhythmia and Electrophysiology,} vol. 5, no. 1, pp. 229--236, 2012.

\bibitem{ng} G. A. Ng, ``Treating patients with ventricular ectopic beats," {\em Heart,} vol. 92, no. 11, pp. 1707--1712, 2006.

%\bibitem{shiraishi} H. Shiraishi, K. Ishibashi, N. Urao, M. Tsukamoto, M. Hyogo, N. Keira, S. Hirasaki, T. Shirayama and M. Nakagawa, ``A case of cardiomyopathy induced by premature ventricular complexes," {\em Circulation journal,} vol. 66, no. 11, pp. 1065-1067, 2002.

%\bibitem{lown} B. Lown and M. Wolf, ``Approaches to sudden death from coronary heart disease," {\em Circulation,} vol. 44, no. 1, pp .130--142, 1971.

\bibitem{poverty} \url{http://data.worldbank.org/indicator/SI.POV.DDAY}

\bibitem{west} D. West, ``How mobile devices are transforming healthcare,'' {\em Issues in technology innovation,} vol. 18, no. 1, pp. 1--11, 2012.

\bibitem{BOP} C. K. Prahalad, {\em The Fortune at the Bottom of the Pyramid,} Pearson Education India, 2006.

\bibitem{frugal} N. Kumar and P. Puranam, ``Frugal engineering: An emerging innovation paradigm," {\em Ivey Business Journal,} vol. 76, no. 2, pp. 14-16, 2012.

\bibitem{perlmutter} K. O. Perlmutter, S. M. Perlmutter, R. M. Gray, R. A. Olshen and K. L. Oehler, ``Bayes risk weighted vector quantization with posterior estimation for image compression and classification," {\em IEEE Transactions on Image Processing,} vol. 5, no. 2, pp. 347--360, 1996.


\bibitem{palreddy} Y. Hu, S. Palreddy and W. J. Tompkins, ``A patient-adaptable ECG beat classifier using a mixture of experts approach," {\em  IEEE Transactions on Biomedical Engineering,} vol. 44, no. 9, pp. 891--900, 1997.

\bibitem{chazal} P. D. Chazal and R. B. Reilly, ``A patient-adapting heartbeat classifier using ECG morphology and heartbeat interval features," {\em IEEE Transactions on Biomedical Engineering,} vol. 53, no. 12, pp. 2535--2543, 2006.


\bibitem{Llamedo} M. Llamedo and J. P. Mart\'{i}nez, ``An automatic patient-adapted ECG heartbeat classifier allowing expert assistance," {\em IEEE Transactions on Biomedical Engineering,} vol. 59, no. 8, pp. 2312--2320, 2012.

\bibitem{melgani} F. Melgani and Y. Bazi, ``Classification of electrocardiogram signals with support vector machines and particle swarm optimization," {\em IEEE Transactions on Information Technology in Biomedicine,} vol. 12, no. 5, pp. 667--677, 2008.


%\bibitem{christov} I. Christov, I. Jekova and G. Bortolan, ``Premature ventricular contraction classification by the Kth nearest-neighbours rule," {\em Physiol. Meas.,} vol. 26, no. 1, 123--130, January 2005.

%\bibitem{chud} V Chud\'{a}\^{c}ek, G. Georgoulas, L. Lhotsk\'{a}, C. Stylios, M. Petrík and M. Čepek, ``Examining cross-database global training to evaluate five different methods for ventricular beat classification", {\em Physiol. Meas.,} vol. 30, no. 7, pp. 661--678, July, 2009.


\bibitem{ince} T. Ince, S. Kiranyaz and M. Gabbouj, ``Automated patient-specific classification of premature ventricular contractions," {\em IEEE Engineering in Medicine and Biology Society,} pp. 5474--5477, 2008.


\bibitem{kiranyaz} S. Kiranyaz, T. Ince and M. Gabbouj, ``Real-Time patient-specific ECG classification by 1D convolutional neural networks," {\em IEEE Transactions on Biomedical Engineering,} vol. 63, no. 3, pp. 664--675, 2016.


\bibitem{bortolan} G. Bortolan, I. Jekova and I. Christov, ``Comparison of four methods for premature ventricular contraction and normal beat clustering," {\em IEEE Computers in Cardiology,} pp. 921--924, 2005.


\bibitem{zzhang} Z. Zhang, J. Dong, X. Luo, K. S. Choi and X. Wu, ``Heartbeat classification using disease-specific feature selection," {\em Computers in biology and medicine,} vol. 46, pp. 79-89, 2014.

\bibitem{jiang} W. Jiang and S. G. Kong, ``Block-based neural networks for personalized ECG signal classification," {\em IEEE Transactions on Neural Networks,} vol. 18, no. 6, pp. 1750--1761, 2007.


%\bibitem{martis} R. J. Martis, U. R. Acharya and L. C. Min, ``ECG beat classification using PCA, LDA, ICA and Discrete Wavelet Transform," {\em Biomedical Signal Processing and Control,} vol. 8, no. 5, pp. 437--448, 2013.


%\bibitem{healthcom} B. S. Chandra, C. S. Sastry and S. Jana, ``Telecardiology: Hurst exponent based anomaly detection in compressively sampled ECG signals," {\em In Proc. of 15th IEEE-Healthcom,} October 2013.


%\bibitem{chazal2} P. D. Chazal, B. G. Celler and R. B. Reilly, ``Using wavelet coefficients for the classification of the electrocardiogram," {\em IEEE Engg. in Med. Bio. Soc.,} pp. 64--67, 2000.
%10 fold cross validation and segmentation 

%\bibitem{kohavi}R. Kohavi, ``A study of cross-validation and bootstrap for accuracy estimation and model selection," {\em Proc. of the Joint Conf. on Artificial Intelligence,} vol. 14, no. 2, 1995.


%\bibitem{velasco} M. Blanco-Velasco, F. Cruz-Rold{\'a}n, J Godino-Llorente, J Blanco-Velasco, C. Armiens-Aparicio and F. L{\'o}pez-Ferreras, ``On the use of PRD and CR parameters for ECG compression," {\em Med. Engg. \& Phy.,} vol. 27, no. 9, pp. 798--802, November 2005.


%\bibitem{zigel} Y. Zigel, A. Cohen, and A. Katz, ``The weighted diagnostic distortion (WDD) measure for ECG signal compression," {\em IEEE Tran. on Biomed. Engg.,} vol. 47, no. 11, pp. 1422-1430, 2000.


%\bibitem{velasco1} M. Blanco-Velasco, F Cruz-Rold{\'a}n, F L{\'o}pez-Ferreras, {\'A} Bravo-Santos and D Mart{\'\i}nez-Mu{\~n}oz, ``A low computational complexity algorithm for ECG signal compression," {\em Med. Engg. \& Phy.,} vol. 26, no. 7, pp. 553--568, September 2004.


\bibitem{tai} S. C. Tai, C. C. Sun and W. C. Yan, ``A 2-D ECG compression method based on wavelet transform and modified SPIHT," {\em IEEE Transactions on Biomedical Engineering,} vol. 52, no. 6, pp. 999--1008, 2005.


%\bibitem{lu} Z. Lu, D. Y. Kim and W. A. Pearlman, ``Wavelet compression of ECG signals by the set partitioning in hierarchical trees algorithm," {\em IEEE Tran. on Biomed. Engg.,} vol. 47, no. 7, pp. 849--856, July 2000.

\bibitem{zigel1} Y. Zigel, A. Cohen, and A. Katz, ``ECG signal compression using analysis by synthesis coding," {\em IEEE Transactions on Biomedical Engineering,} vol. 47, no. 10, pp. 1308--1316, 2000.


%\bibitem{kanoun} K. Kanoun, H. Mamaghanian, N. Khaled and D. Atienza, ``A real-time compressed sensing-based personal electrocardiogram monitoring system," {\em Design, Automation \& Test in Europe Conference \& Exhibition,} pp. 1--6, March 2011.


\bibitem{fira1} C. M. Fira and L. Goras, ``An ECG signals compression method and its validation using NNs," {\em IEEE Transactions on Biomedical Engineering,} vol. 55, no. 4, pp. 1319--1326, 2007.

\bibitem{adamo} A. Adamo, G. Grossi, R. Lanzarotti and J. Lin, ``ECG compression retaining the best natural basis k-coefficients via sparse decomposition," {\em Biomedical Signal Processing and Control,} vol. 15, pp. 11--17, 2015.

\bibitem{jana} S. Jana and P. Moulin, ``Optimality of KLT for high-rate transform coding of gaussian vector-scale mixtures: application to reconstruction, estimation, and classification," {\em IEEE Transactions on Information Theory,} vol. 52, no. 9, pp. 4049--4067, 2006.

%\bibitem{lee} S. J. Lee, J. Luan and P. H. Chou, ``A new approach to compressing ECG signals with trained overcomplete dictionary," {\em Int. conf. on Wireless Mobile Comm. and Healthcare,} pp. 83--86, 2014.

\bibitem{vlodaver} Z. Vlodaver, R. F. Wilson and D. J. Garry, {\em Coronary Heart Disease: Clinical, Pathological, Imaging, and Molecular Profiles,} Springer Science \& Business Media, 2012.

\bibitem{niwano} S. Niwano, Y. Wakisaka, H. Niwano, H. Fukaya, S. Kurokawa, M. Kiryu, Y. Hatakeyama and T. Izumi, ``Prognostic significance of frequent premature ventricular contractions originating from the ventricular outflow tract in patients with normal left ventricular function," {\em Heart,} vol. 95, no. 15, pp. 1230--1237, 2009.

\bibitem{baman} T. S. Baman, D. C. Lange, K. J. Ilg, S. K. Gupta, T. Y. Liu, C. Alguire, W. Armstrong, E. Good, A. Chugh, K. Jongnarangsin and F. Pelosi, ``Relationship between burden of premature ventricular complexes and left ventricular function," {\em Heart Rhythm,} vol. 7, no. 7, pp. 865--869, 2010.

\bibitem{scheidt} S. Scheidt, J. McGill, G. Wilner and T. Killip, ``Remote electrocardiography: clinical experience with telephone transmission of electrocardiograms," {\em JAMA,} vol. 230, no. 9, pp. 1293--1294, 1974.

\bibitem{varshney} U. Varshney, ``Pervasive healthcare," {\em Computer,} vol. 36, no. 12, pp. 138--140, 2003.

\bibitem{huang} A. Huang, C. Chen, K. Bian, X. Duan, M. Chen, H. Gao, C. Meng, Q. Zheng, Y. Zhang, B. Jiao and L. Xie, ``WE-CARE: an intelligent mobile telecardiology system to enable mHealth applications," {\em IEEE Journal of Biomedical and Health Informatics,} vol. 18, no. 2, pp. 693--702, 2014.


\bibitem{leehj} H. J. Lee, S. H. Lee, K. S. Ha, H. C. Jang, W. Y. Chung, J. Y. Kim, Y. S. Chang and D. H. Yoo, ``Ubiquitous healthcare service using Zigbee and mobile phone for elderly patients, {\em International Journal of Medical Informatics,} vol. 78, no. 3, pp. 193--198, 2009.

\bibitem{Mukhopadhyay} S. K. Mukhopadhyay, S. Mitra and M. Mitra, ``A lossless ECG data compression technique using ASCII character encoding," {\em Computers and Electrical Engineering} vol. 37, no. 4, pp. 486--497, 2011.

%\bibitem{Med} M. S. Thaler, {\em The Only EKG Book You'll Ever Need}, 5th ed. Philadelphia, PA: Lippincott Williams \& Wilkins, 2007.


\bibitem{ICT} W. H. Lehr, {\em Quality and Reliability of Telecommunications Infrastructure,} Routledge, 2013.

\bibitem{steg} P. G. Steg, S. K. James, D. Atar, L. P. Badano, C. B. Lundqvist, M. A. Borger, C. Di Mario, K. Dickstein, G. Ducrocq, F. Fernandez-Aviles and A. H. Gershlick, ``ESC Guidelines for the management of acute myocardial infarction in patients presenting with ST-segment elevation," {\em European heart journal,} pp. ehs215, 2012. 

\bibitem{purohit} B. C. Purohit, ``Private initiatives and policy options: recent health system experience in India," {\em Health policy and planning,} vol. 16, no. 1, pp. 87--97, 2001.


\bibitem{jarosławski} S. Jarosławski and G. Saberwal, ``In eHealth in India today, the nature of work, the challenges and the finances: an interview-based study," {\em BMC medical informatics and decision making,} vol. 14, no. 1, pp. 1, 2014.


\bibitem{physionet} A. L. Goldberger, L. A. N. Amaral, L. Glass, J. M. Hausdorff, P. Ch. Ivanov, R. G. Mark, J. E. Mietus, G. B. Moody, C. K. Peng and H. E. Stanley, ``PhysioBank, PhysioToolkit, and PhysioNet: Components of a new research resource for complex physiologic signals," {\em Circulation,} vol. 101, no. 23, pp. e215--e220, 2000.


\bibitem{affordability} L. M. Ni{\"e}ns, E. Van de Poel, A. Cameron, M. Ewen, R Laing and W. B. F. Brouwer, W.B.F., ``Practical measurement of affordability: an application to medicines," {\em Bulletin of the World Health Organization,} vol. 90, no. 3, pp. 219--227.

\bibitem{household} \url{http://www.nakono.com/tekcarta/databank/households-average-household-size}

\bibitem{NP} J. Neyman and E. S. Pearson, ``On the problems of the most efficient tests of statistical hypotheses," {\em Philosophical Transactions of the Royal Society of London,} 1933.

\bibitem{sornmo} L. S{\"o}rnmo and P. Laguna, {\em Bioelectrical signal processing in cardiac and neurological applications,} Elsevier Academic Press, 2005.

\bibitem{wdd} Y. Zigel, A. Cohen and A. Katz, ``The weighted diagnostic distortion (WDD) measure for ECG signal compression," {\em IEEE Transactions on Biomedical Engineering,} vol. 47, no. 11, pp. 1422--1430, 2000.

%\bibitem{kanei} Y. Kanei, M. Friedman, N. Ogawa, S. Hanon, P. Lam and P. Schweitzer, ``Frequent premature ventricular complexes originating from the right ventricular outflow tract are associated with left ventricular dysfunction," {\em Annals of Noninvasive Electrocardiology,} vol. 13, no. 1, pp. 81--85, 2008.


%\bibitem{baman} T. S. Baman, D. C. Lange, K. J. Ilg, S. K. Gupta, T. Y. Liu, C. Alguire, W. Armstrong, E. Good, A. Chugh, L. Jongnarangsin and F. Pelosi, ``Relationship between burden of premature ventricular complexes and left ventricular function, {\em Heart Rhythm,} vol. 7, no. 7, pp. 865--869, 2010.

%\bibitem{ruberman} W. Ruberman, E. Weinblatt, J. D. Goldberg, C. W. Frank and S. Shapiro, ``Ventricular premature beats and mortality after myocardial infarction," {\em New England Journal of Medicine,} vol. 297, no. 14, pp.750--757, 1977.


%\bibitem{katritsis} D. G. Katritsis, G. C. Siontis and A. J. Camm, ``Prognostic significance of ambulatory ECG monitoring for ventricular arrhythmias," {\em Progress in cardiovascular diseases,} vol. 56, no. 2, pp. 133--142, 2013.

%\bibitem{ephrem} G. Ephrem, M. Levine, P. Friedmann and P. Schweitzer, ``The prognostic significance of frequency and morphology of premature ventricular complexes during ambulatory holter monitoring," {\em Annals of Noninvasive Electrocardiology,} vol. 18, no. 2, pp. 118--125, 2013. 

%\bibitem{ahn} M. S. Ahn, ``Current Concepts of Premature Ventricular Contractions," {\em Journal of Lifestyle Medicine,} vol. 3, no. 1, pp. 26-33, 2013.


%\bibitem{physician} \url{http://data.worldbank.org/indicator/SH.MED.PHYS.ZS}


%\bibitem{atsushi} I. Atsushi, M. Hwa, A. Hassankhani, T. Liu, and S. M. Narayan, ``Abnormal heart rate turbulence predicts the initiation of ventricular arrhythmias," {\em Pacing Clinical Electrophysiology,} vol. 11, pp. 1189--1197, 2005.

%\bibitem{schneider} R. Schneider, P. Barthel, and M. Watanabe, ``Heart rate turbulence on holter," {\em Dynamic Electrocardiography,} pp. 190--193, 2004.




%\bibitem{kreutz} K. Kreutz-Delgado, J. F. Murray, B. D. Rao, K. Engan, T. W. Lee and T. J. Sejnowski, ``Dictionary learning algorithms for sparse representation," {\em Neural computation,} vol. 15, no. 2, pp. 349--396, 2003.

%\bibitem{rubinstein} R. Rubinstein, A. M. Bruckstein and M. Elad, ``Dictionaries for sparse representation modeling," {\em Proceedings of the IEEE,} vol. 98, no. 6, pp. 1045--1057, 2010.

%\bibitem{ramirez}I. Ramirez, P. Sprechmann and G. Sapiro, ``Classification and clustering via dictionary learning with structured incoherence and shared features," {\em IEEE Conference on Computer Vision and Pattern Recognition}, pp. 3501--3508, 2010.

%\bibitem{fang} Q. Fang, F. Sufi and I. Cosic, {\em A mobile device based ECG analysis system,} INTECH Open Access Publisher, 2008.



%\bibitem{telecardiology} P. Sekar and V. Vilvanathan, ``Telecardiology: effective means of delivering cardiac care to rural children." {\em Asian Cardiovascular and Thoracic Annals,} vol. 15, no. 4, pp. 320--323, 2007.

%\bibitem{baig} M. M. Baig and H. Gholamhosseini, ``Smart health monitoring systems: an overview of design and modeling," {\em Journal of medical systems,} vol. 37, no. 2, pp. 1--14, 2013.


%\bibitem{leerg} R. G. Lee, K. C. Chen, C. C. Hsiao and C. L. Tseng, ``A mobile care system with alert mechanism," {\em IEEE Transactions on Information Technology in Biomedicine,} vol. 11, no. 5, pp. 507--517, 2007.



\bibitem{elad} M. Elad, {\em Sparse and redundant representations: from theory to applications in signal and image processing,} Springer Science \& Business Media, 2010.


\bibitem{ksvd} M. Aharon, M. Elad and A. Bruckstein, ``K-SVD: An algorithm for designing overcomplete dictionaries for sparse representation," {\em IEEE Transsactions on Signal Processing,} vol. 54, no. 11, 2006.

\bibitem{ye} C. Ye, B. V. Kumar and M. T. Coimbra, ``Heartbeat classification using morphological and dynamic features of ECG signals," {\em IEEE Transactions on Biomedical Engineering,} vol. 59, no. 10, pp. 2930--2941, 2012.


\bibitem{krasteva} V. Krasteva and I. Jekova, ``QRS Template Matching for Recognition of Ventricular Ectopic Beats," {\em Annals of Biomedical Engineering}, vol. 35, no. 12, pp. 2065--2076, 2007.

%\bibitem{Llamedo1} M. Llamedo and J. P. Mart\'{i}nez, ``Heartbeat classification using feature selection driven by database generalization criteria," {\em IEEE Transactions on Biomedical Engineering,} vol. 58, no. 3, pp.616--625, 2011;

\bibitem{MCCV} S. Arlot and A. Celisse, ``A survey of cross-validation procedures for model selection," {\em Statistics surveys,} vol. 4, pp. 40--79, 2010.

\bibitem{HC14} B. S. Chandra, C. S. Sastry and S. Jana, ``Reliable low-cost telecardiology: High-sensitivity detection of ventricular beats using dictionaries," {\em IEEE 16th international conference on e-health networking, applications and services,} pp. 305--310, 2014.

\bibitem{aami} Testing and Reporting Performance Results of Cardiac Rhythm and ST Segment Measurement Algorithms, ANSI/AAMI EC57:1998 standard, Association for the Advancement of Medical Instrumentation, 1998.

%Recommended Practice for Testing and Reporting Performance Results of Ventricular Arrhythmia Detection Algorithms Association for the Advancement of Medical lnstrumentation, Arlington, VA, 1987, ANSI ECAR:1987.



%\bibitem{bhushan} M. Bhushan and S. J. Asirvatham, ``The conundrum of ventricular arrhythmia and cardiomyopathy: which abnormality came first?," {\em Current heart failure reports,} vol. 6, no. 1, pp. 7--13, 2009.

%\bibitem{blaauw} Y. Blaauw, L. Pison, J. M. van Opstal, R. M. Dennert, W. F. Heesen and H. J. G. M. Crijns, ``Reversal of ventricular premature beat induced cardiomyopathy by radiofrequency catheter ablation," {\em Netherlands Heart Journal,} vol. 18, no. 10, pp. 493--498, 2010.



%\bibitem{cui} C. Li, C. Zheng and C Tai, ``Detection of ECG characteristic points using wavelet transforms," {\em IEEE Trans. in Biomed. Engg.,} vol. 42, no. 1, pp. 21--28, January 1995.

%\bibitem{ran} P. Ranjith, P. C. Baby and P. Joseph, ``ECG analysis using wavelet transform: application to myocardial ischemia detection," {\em Innovation and Research in Biomed. Engg,} vol. 24, no. 1, pp. 44--47, February 2003.

%\bibitem{zhang} D. Zhang, G. Tan and J. Hao, ``Fractal random walk and classification of ECG signal," {\em Int. J. of Hybrid Inform. Technology,} vol. 1, no. 1,  pp. 1--10, January 2008.


%\bibitem{pao} P. B. DePetrillo and U. E. Ruttimann, ``Determining the Hurst exponent of fractal time series and its application to electrocardiographic analysis." {\em Comp. in bio. and med.} vol. 29, no. 6, pp. 393--406, November 1999.

%\bibitem{Jiang} W. Jiang, S. G. Kong and G. D. Peterson, ``ECG signal classification using block-based neural networks," {\em IEEE Int. Joint Conf. on Neural Networks,} vol. 1, pp. 326--331, August 2005.

%\bibitem{comp2} M. Fira, L. Goras, N. Cleju and C. Barbasa, `` On the projection matrices influence in the classification of compressed sensed ECG signals," {\em Int. J. of Adv. Comp. Science and Applications,} vol. 3, no. 8, 2012. 

%\bibitem{comp1} H. Ding, H. Sun and Kun-mean Hou, ``Abnormal ECG signal detection based on Compressed Sampling in Wearable ECG sensor,"  {\em  Int. Conf. on Wireless Comm. and Sig. Proc.,} pp. 1--5, November 2011.

%\bibitem{elad} M. Elad, {\em Sparse and Redundant Representations: From Theory to Applications in Signal and Image Processing,} New York: Springer, 2010.



%\bibitem{bdr} K. K. Delgado, J. F. Murray, B. D. Rao, K. Engan, T. Lee, and T. J. Sejnowski. ``Dictionary learning algorithms for sparse representation." {\em Neural computation,} vol. 15, no. 2, pp. 349--396, 2003.

%\bibitem{ecgbook}  M. S. Thaler, {\em The only EKG book you'll ever need,} Lippincott Williams \& Wilkins, 2010.

%\bibitem {ID} I. Daubechies, {\em Ten lectures on wavelets,} CBMS-NSF Series in Appl. Math. vol. 61, SIAM, Philadelphia, 1992.


%\bibitem{abry} P. Abry and D. Veitch, ``Wavelet analysis of long-range dependent traffic," {\em IEEE Trans. Inform. Theory,} vol. 44, no. 1, pp. 2--15, January 1998.


%\bibitem {gilbert2001} A. C. Gilbert, ``Multiscale Analysis and Data Networks," {\em Applied and Computational Harmonic Analysis}, Vol. 10, pp: 185-202, 1992.


%\bibitem{taqqu} S. Stoev, M. Taqqu, C. Park, J.S. Marron, ``On the wavelet spectrum diagnostic for Hurst parameter estimation in the analysis of Internet traffic," {\em Computer Networks}, Vol. 48, pp: 423-445, 2005.


%\bibitem{amit} E. B. Mazomenos, D. Biswas, A. Acharyya, T. Chen, K. Maharatna, J. Rosengarten, J. Morgan and N. Curzen, ``A low-complexity ECG feature extraction algorithm for mobile healthcare applications," {\em IEEE J. of Biomed. and health informatics,} vol. 17, no. 2, pp. 459--469, March 2013.

%\bibitem{NCHS} National Center for Health Statistics (NCHS). Summary health statistics for U.S. adults: National Health Interview Survey, 2012. Vital Health Stat. 10(260). \url{ http://www.cdc.gov/nchs/data/series/sr_10/sr10_260.pdf.}


%\bibitem{ref1} A J Moss, H T Davis, J DeCamilla, and L W Bayer, ``Ventricular ectopic beats and their relation to sudden and nonsudden cardiac death after myocardial infarction," {\em Circulation,} vol. 60 no. 5  pp. 998-1003, 1979.

%\bibitem{chow} H. S. Chow, G. B. Moody and R. G. Mark, ``Detection of ventricular ectopic beats using neural networks," {\em Comp. in Cardiology}, pp. 659--662, 1992.


%\bibitem{maheshwari} S. Maheshwari, A. Acharyya, P. Rajalakshmi, P. E. Puddu and M. Schiariti, ``Accurate and reliable 3-Lead to 12-Lead ECG reconstruction methodology for remote health monitoring applications," {\em IEEE Healthcom,} pp. 233--237, October 2013.

%\bibitem{healthcom14} B. S. Chandra, C. S. Sastry, S. Jana, ``Reliable low-cost telecardiology: High-sensitivity detection of ventricular beats using dictionaries," {\em IEEE Healthcom,} pp. 305--310, October 2014.


%\bibitem{healthcom14} B. S. Chandra, C. S. Sastry and S. Jana, ``Reliable low-Cost telecardiology: High-sensitivity detection of ventricular beats using dictionaries," {\em IEEE-Healthcom,} October, 2014. 

%\bibitem{jana} S. Jana and P Moulin, ``Optimal transform coding of Gaussian mixtures for joint classification/reconstruction." {\em Proceedings of IEEE Data Compression Conf.,} 2003.



%\bibitem{kastania} A. N. Kastania, S. Demarias, C. Davos, C. Boudoulas and S. Kossida, ``A telecardiology service quality model," {\em In Proc. of the Int. Educational and Networking Forum for eHealth, Telemedicine and Health ICT,} pp. 173--176, 2007.

%\bibitem{argulian}E. Argulian, D. G. Halpern, E. F. Aziz and E. Herzog, 2012. Supraventricular Arrhythmias and Atrial Fibrillation. The Cardiac Care Unit Survival Guide, p.170.


\bibitem{amatriain} X. Amatriain, A. Jaimes, N. Oliver and J. M. Pujol, {\em Data mining methods for recommender systems,} In Recommender Systems Handbook, pp. 39-71, Springer US, 2011


\bibitem{page} R. L. Page, W. E. Wilkinson, W. K. Clair, E. A. McCarthy and E. L. Pritchett, ``Asymptomatic arrhythmias in patients with symptomatic paroxysmal atrial fibrillation and paroxysmal supraventricular tachycardia," {\em Circulation,} vol. 89, no. 1, pp. 224--227, 1994.


\bibitem{mairal} J. Mairal,  F. Bach, J. Ponce and G. Sapiro, ``Online dictionary learning for sparse coding," {\em In Proceedings of the 26th annual international conference on machine learning,} pp. 689--696, ACM, 2009.


%\bibitem{amit} S. Maheshwari, A. Acharyya, P. Rajalakshmi, P. E. Puddu and M. Schiariti, ``Accurate and reliable 3-lead to 12-lead ECG reconstruction methodology for remote health monitoring applications," {\em Innovation and Research in Biomedical Engineering, Elsevier,} vol. 35, no. 6, pp. 341-350, 2014.

%\bibitem{menz} M. D. Menz and D. Michael, ``Minimum Sampling Rate in Electrocardiology," {\em J. of Clinical Engg.,} vol. 19, no. 5, 1994.

%\bibitem{aufderheide} T. P. Aufderheide, G. E. Hendley, R. K. Thakur, J. R. Mateer, H. A. Stueven, D. W. Olson, K. M. Hargarten, F. Laitinen, N. Robinson, K. C. Preuss and R. G. Hoffman, ``The diagnostic impact of prehospital 12-lead electrocardiography," {\em Annals of emergency medicine,} vol. 19, no. 11, pp. 1280--1287, 1990.

%\bibitem{bedi} B. S. Bedi, ``Telemedicine standards: need and Indian initiatives," {\em Telemedicine and e-Health,} vol. 15, no. 6, pp. 597--599, 2009.

%\bibitem{gough} F. Gough, S. Budhrani, E. Cohn, A. Dappen, C Leenknecht, B. Lewis, D. A. Mulligan, D. Randall, K. Rheuban, L. Roberts, T. J. Shanahan, K. Webster and J. Bernard, ``ATA Practice Guidelines for Live, On-Demand Primary and Urgent Care," {\em Telemedicine and e-Health,} vol. 21, no. 3, pp. 233-241, 2015.



%\bibitem{amit} S. Maheswari, A. Acharyya, P. E. Puddu and M. Schiariti, ``Reduced lead system selection methodology for reliable standard 12-lead reconstruction targeting personalised remote health monitoring applications," {\em Computer Methods in Biomechanics and Biomedical Engineering: Imaging \& Visualization,} vol. 2, no. 2, pp. 107--120, 2014.


%\bibitem{engel} G. Engel, S. Cho, A. Ghayoumi, T. Yamazaki, S. Chun, W. F. Fearon and V. F. Froelicher, ``Prognostic significance of PVCs and resting heart rate," {\em Annals of Noninvasive Electrocardiology,} vol. 12, no. 2, pp. 121--129, 2007.








%\bibitem{gomez} G. G\'{o}mez-Herrero, I. Jekova, V. Krasteva, I. Christov, A. Gotchev, and K. Egiazarian, ``Relative estimation of the Karhunen-Lo\`{e}ve transform basis functions for detection of ventricular ectopic beats.", {\em IEEE Comp. in Cardiology,} pp. 569--572, 2006.

%\bibitem{charles} L. F. Charles, P. G. Amazeen, D. K. Michael, L. Bernard, ``Computer detection of ventricular ectopic beats", {\em Computers and Biomedical Research,} vol. 3, no. 6, pp. 666--674, 1970.

%\bibitem{wiens} Wiens, J.; Guttag, John V.,``Patient-specific ventricular beat classification without patient-specific expert knowledge: A transfer learning approach," {\em  Engineering in Medicine and Biology Society,} pp.5876--5879, 2011.




%\bibitem{mccutecheon} K. McCutcheon, K. M. A. Rogers, ``The principles and practice of interpreting cardiac rhythm strips: a seven-step model", {\em Journal of Perioperative Practice,} vol 24, no 2, pp. 19--24, 2014.

%\bibitem{tadejko} P. Tadejko, W. Rakowski,``Mathematical Morphology Based ECG Feature Extraction for the Purpose of Heartbeat Classification," {\em Computer Information Systems and Industrial Management Applications,} pp.322--327, June 2007.

%\bibitem{taccardi} B Taccardi, G Arisi, E Macchi, S Baruffi, and S Spaggiari, ``A new intracavitary probe for detecting the site of origin of ectopic ventricular beats during one cardiac cycle", {\em Circulation,}  vol. 75, no. 1, pp. 272--281, 1987.


%\bibitem{hu} Y. Hu, W. J. Tompkins, J. L. Urrusti, and V. X. Afonso, ``Applications of Artificial Neural Networks for ecg Signal Detection and Classification," {\em Journal of Electrocardiology,} vol. 26, pp. 66--73, 1993. 


%\bibitem{inan} O. T. Inan, L. Giovangrandi and G. T. A. Kovacs, ``Robust neural-network-based classification of premature ventricular contractions using wavelet transform and timing interval  features," {\em IEEE Tran. on Biomed. Engg.,} vol. 53, no. 12, pp. 2507--2515, December 2006.


\end{thebibliography}
